Lower-Left Partial AUC: An Effective and Efficient Optimization Metric for Recommendation

Optimization metrics are crucial for building recommendation systems at scale. However, an effective and efficient metric for practical use remains elusive. While Top-K ranking metrics are the gold standard for optimization, they suffer from significant computational overhead. Alternatively, the more efficient accuracy and AUC metrics often fall short of capturing the true targets of recommendation tasks, leading to suboptimal performance. To overcome this dilemma, we propose a new optimization metric, Lower-Left Partial AUC (LLPAUC), which is computationally efficient like AUC but strongly correlates with Top-K ranking metrics. Compared to AUC, LLPAUC considers only the partial area under the ROC curve in the Lower-Left corner to push the optimization focus on Top-K. We provide theoretical validation of the correlation between LLPAUC and Top-K ranking metrics and demonstrate its robustness to noisy user feedback. We further design an efficient point-wise recommendation loss to maximize LLPAUC and evaluate it on three datasets, validating its effectiveness and robustness.

==> sections/7_Limitation.tex <==
We agree that strictly speaking, if we want to obtain the best Top-K performance with specific K, different users should enjoy different $\alpha$ and $\beta$. However, we argue that, in practical application, it’s already enough to use the same $\alpha$ and $\beta$ for all users, which is also verified by our empirical results. Due to the data sparsity shown in Appendix H.1, for all datasets, $\frac{\Delta n_-}{n_-}\approx 0.001$. For $n_+$, we report the percentage statistics of $n_+$ of users on all datasets in Rebuttal Figure 9. From it, we can also observe that the majority of users have a small gap in $n_+$. Hence, specific Top-K metrics can be approximately optimized using the same $\alpha$ and $\beta$ for all users. For further work, we'll explore how to use user-specific $\alpha$ and $\beta$ to achieve better performance.
